Bridging the Gap between Programming Languages and Hardware Weak Memory Models

We develop a new intermediate weak memory model, IMM, as a way of modularizing the proofs of correctness of compilation from concurrent programming languages with weak memory consistency semantics to mainstream multi-core architectures, such as POWER and ARM. We use IMM to prove the correctness of compilation from the promising semantics of Kang et al. to POWER (thereby correcting and improving their result) and ARMv7, as well as to the recently revised ARMv8 model. Our results are mechanized in Coq, and to the best of our knowledge, these are the first machine-verified compilation correctness results for models that are weaker than x86-TSO.

==> cert-old.tex <==
\subsection{A certification related execution transformation}
\label{sec:cert}

\begin{definition}
An execution $G'$ is a \emph{prefix} of an execution $G$, denoted $\prefix(G',G)$,
if the following hold:
\begin{itemize}
\item $G'.\lE \suq G.\lE$
\item $G'.\lLAB = \restr{G.\lLAB}{G'.\lE}$
%% \item $G'.\lPO \suq G.\lPO$ \ori{we need to decide whether we need/want $\lPO$ as a part of $G$}
\item $G'.\lRF \suq G.\lRF$
\item $G'.\lCO \suq G.\lCO$
\item $G'.\lRMW \suq G.\lRMW$
\item $G'.\lCTRL \suq G.\lCTRL$
\item $G'.\lADDR \suq G.\lADDR$
\item $G'.\lDATA \suq G.\lDATA$
\item $\dom{G.\lPO; [G'.\lE]} \suq G'.\lE$
\end{itemize}
\end{definition}

\begin{definition}
Let $\tup{\CoveredSet,\IssuedSet}$ be a traversal configuration for an execution $G$.
The set of \emph{determined} events by $\tup{C,I}$ in $G$, denoted $\determined(G,\CoveredSet,\IssuedSet)$,
is given by
$$\determined(G,\CoveredSet,\IssuedSet)\defeq
\CoveredSet \cup \dom{G.\lDETOUR^?; (G.\lDEPS \cup G.\lRFI)^*; [\IssuedSet]}.$$
\end{definition}


$\complRel(\Cf, G)$ states that graph $G$ is an execution of program $\Cf$:

$$\complPrefixRel(\Cf, G') \defeq  \consistent(G') \land \exists G.\; \complRel(\Cf, G) \land \prefix(G',G) $$


\[\inarr{
\certCompl(G, \tup{\CoveredSet, \IssuedSet}, G') \defeq {} \\
\quad \letdef{D}{\determined(G,\CoveredSet,\IssuedSet)} \\
\quad D \suq G'.\lE \suq G.\lE \land \restr{G'.\lLAB}{D} = \restr{G.\lLAB}{D} \land {} \\
\quad % G'.\lPO = [G'.\lE]; G.\lPO; [G'.\lE] \land
      G'.\lE \suq \dom{G'.\lPO^?; [D]} \land {} \\
\quad G'.\lCTRL = [G'.\lE]; G.\lCTRL; [G'.\lE] \land {} \\
%% \quad G'.\lADDR; [D] = G.\lADDR; [D] \land {} \\
%% \quad G'.\lDATA; [D] = G.\lDATA; [D] \land {} \\
\quad G'.\lADDR; [D] = G.\lADDR; [D] \land {} \\
\quad G'.\lDATA; [D] = G.\lDATA; [D] \land {} \\
\quad [D]; G'.\lCO; [D] = [D]; G.\lCO; [D] \land {} \\
\quad G'.\lRF; [D] = G.\lRF; [D] \land {} \\
\quad (\forall r \in G'.\lR \setminus D. \\
\qquad G'.\lRF^{-1}(r) =
      {\rm \bf max}_{G'.\lCO}(G'.\lW_{\lLOC(r)} \cap \dom{G'.\lPO; [r] \cup G'.\curRel; [\CoveredSet^{\lTID(r)}]}))
  \land {} \\
%% G'.\lRF; [G'.\lE \setminus D] \suq G'.\curRel; G'.\lPO 
\quad G'.\lRMW = G.\lRMW; [D] \land {} \\
\quad (\forall w \in G'.\lE \setminus D. \\
\qquad [w]; G'.\lCO; [D] = \emptyset \lor {} \\
\qquad \exists w' \in G'.\lW. \; \tup{w, w'} \in G'.\lCOI \setminus (G'.\lCO; G'.\lCO)). \\

%% [w]; G'.\lCOI; [D] = \emptyset \Rightarrow [w]; G'.\lCO; [D] = \emptyset).
%% \quad [G'.\lE \setminus D]; G'.\lCOI \cap G'.\lCOE; G'.\lCOE = \emptyset \land {} \\
}\]


\begin{lemma}
\label{prop:cert-compl}
  Suppose that
  $\complRel(\Cf, G)$ and $\travConfig(G, \tup{\CoveredSet, \IssuedSet})$
  hold.
  Then there exists $G'$ s.t. $\travConfig(G', \tup{\CoveredSet, \IssuedSet})$,
  $\complPrefixRel(\Cf, G')$, and $\certCompl(G, \tup{\CoveredSet, \IssuedSet}, G')$ hold.
\end{lemma}

\begin{lemma}
\label{prop:cert-compl-consist}
  Suppose that
  $\phConsistent(G)$, $\travConfig(G, \tup{\CoveredSet, \IssuedSet})$, and $\certCompl(G, \tup{\CoveredSet, \IssuedSet}, G')$ hold.
  Then $\phConsistent(G')$ holds.
\end{lemma}

\[\inarr{
  \certMemTwo(G, \Tto, \Tfrom, \CoveredSet, \IssuedSet, M) \defeq \forall m \in M. \; \\
  \quad (\forall tid. \; m \in \TSf(tid).\PromSet \Rightarrow \\
  \qquad \exists w \in \IssuedSet \setminus \CoveredSet. \;
     G.\lTID(w) = tid \land \sameMsgEvent(G, \Tto, \Tfrom, m, w)) \land {} \\
  \quad ((\forall w \in G.\lE. \; (m.{\rm from}, m.{\rm to}] \cap (\Tfrom(w), \Tto(w)] = \emptyset) \lor {} \\
  \quad \; \; \, \exists w \in \IssuedSet. \; \sameMsgEvent(G, \Tto, \Tfrom, m, w)). \\
  \\
  \certRel(G, \Tto, \Tfrom, \CoveredSet, \IssuedSet, \TSf, M) \defeq
       \simRelBase(G, \Tto, \Tfrom, \CoveredSet, \IssuedSet, \TSf, M) \land {} \\
  \quad \certMemTwo(G, \Tto, \Tfrom, \CoveredSet, \IssuedSet, \TSf, M). \\
}\]

\begin{lemma}
  \label{prop:simrel-to-certrel}
  Suppose that $\simRel(G, \Tto, \Tfrom, \CoveredSet, \IssuedSet, \TSf, \SCview, M)$ holds and $M'$ is a future memory to $M$.
  %% and $\SCview' \sqsupseteq \SCview$.
  Then there exist $G', \Tto', \Tfrom'$ s.t. $\certCompl(G, \tup{\CoveredSet, \IssuedSet}, G')$ and
    $\certRel(G',  \Tto', \Tfrom', \CoveredSet, \IssuedSet, \TSf, M')$ hold.
\end{lemma}

\begin{lemma}
  \label{prop:simrel-step}
  Suppose that $\certRel(G, \Tto, \Tfrom, \CoveredSet, \IssuedSet, \TSf, M)$, $tid \in \dom{\TSf}$, and $\TSf(tid).\PromSet \neq \emptyset$ hold.
  Then, for every $\SCview$, there exist $\TS'$, $M'$, $\CoveredSet''$, $\IssuedSet''$, and $e$ s.t. 
  $G.\lTID(e) = tid$,
  $\tup{\TSf(tid), \SCview, M} \stepp \tup{\TS', \SCview, M'}$,
  $G \vdash \tup{\CoveredSet, \IssuedSet} \travConfigStep^{*}
    \tup{\CoveredSet'' \cup \{e\}, \IssuedSet''}$, and
  $\certRel(G, \Tto, \Tfrom, \CoveredSet'', \IssuedSet'', \TSf[tid \mapsto \TS'], M')$.
\end{lemma}

\begin{lemma}
  \label{prop:cert-thm}
  Suppose that $\simRel(G, \Tto, \Tfrom, G.\lE, G.\lW, \TSf, \SCview, M)$, $tid \in \dom{\TSf}$,
  $\SCview' \ge \SCview$, and $M'$ is a future memory to $M$.
  Then there exists $\TS''$ and $M''$ s.t.:
  \begin{itemize}
  \item $\tup{\TSf(tid), \SCview', M'} \stepp^{*} \tup{\TS'', \SCview', M''}$, and
  \item $\TS''.\PromSet = \emptyset$.
  \end{itemize}
\end{lemma}
\begin{proof}
  We start by applying \cref{prop:simrel-to-certrel}.
  Thus we know that there are $G'$, $\Tto'$, and $\Tfrom'$ s.t. \\
  $\certCompl(G, \tup{\CoveredSet, \IssuedSet}, G')$ and
    $\certRel(G',  \Tto', \Tfrom', \CoveredSet, \IssuedSet, \TSf, M')$.
  We have $|\TSf(tid)| \le |(\IssuedSet \setminus \CoveredSet) \cap G'.\lE_{tid}|$,
  because $\certMemTwo(G',  \Tto', \Tfrom', \CoveredSet, \IssuedSet, \TSf, M')$ holds.
  By applying \cref{prop:simrel-step} $|(\IssuedSet \setminus \CoveredSet) \cap G'.\lE_{tid}|$ times,
  we construct $\TS''$ and $M''$ s.t.
  $\certRel(G',  \Tto', \Tfrom', \CoveredSet \cup G'.\lE_{tid}, \IssuedSet \cup G'.\lW_{tid}, \TSf[tid \mapsto \TS''], M'')$.
  We have $\TS''.\PromSet = \emptyset$,
  because $\certMemTwo(G',  \Tto', \Tfrom', \CoveredSet  \cup G'.\lE_{tid}, \IssuedSet  \cup G'.\lW_{tid}, \TSf[tid \mapsto \TS''], M'')$ holds.
\end{proof}

\subsection{Auxiliary lemmas about $\certCompl$}
In all following lemmas we assume that 
  $\phConsistent(G)$, $\travConfig(G, \tup{\CoveredSet, \IssuedSet})$, $\CoveredSet \suq \coverable(G, \CoveredSet, \IssuedSet)$,
  $\IssuedSet \suq \issuable(G, \CoveredSet, \IssuedSet)$, $\relWriteCovering(G, \CoveredSet, \IssuedSet)$,
  $\rmwCovering(G, \CoveredSet)$, and $\certCompl(G, \tup{\CoveredSet, \IssuedSet}, G')$ hold.

\begin{lemma}
  \label{prop:acq-in-cov}
  $G'.\lE^{\sqsuq \acq} \suq \CoveredSet$.
\end{lemma}
\begin{proof}
  Fix $e \in G'.\lE^{\sqsuq \acq}$. We have $e \in \dom{G'.\lPO^?; [D]}$, because $\certCompl(G, \tup{\CoveredSet, \IssuedSet}, G')$.
  That $e \in \dom{G.\lPO^?; [\CoveredSet]} \cup \dom{G.\lPO^?; [\IssuedSet]}$ follows from it.
  If $e \in \dom{G.\lPO^?; [\CoveredSet]}$, then $e \in \CoveredSet$ since $\CoveredSet$ is $\lPO$-prefix-closed by
  $\travConfig(G, \tup{\CoveredSet, \IssuedSet})$.
  If $e \in \dom{G.\lPO^?; [\IssuedSet]}$, then $e \in \CoveredSet$ since $\IssuedSet \suq \issuable(G, \CoveredSet, \IssuedSet)$
  and $[e]; G.\lPO; [\lW] \suq [G'.\lE^{\sqsuq \acq}]; G.\lPO; [\lW] \suq G.\lBOB$.
\end{proof}

\begin{lemma}
  \label{prop:acq-in-cov}
  $G'.\lF^{\sqsuq \rel} \suq \CoveredSet$.
\end{lemma}
\begin{proof}
  The same proof as in \cref{prop:acq-in-cov}.
\end{proof}

\begin{lemma}
  \label{prop:rel-fence-in-cov}
  $G'.\lF \suq \CoveredSet$.
\end{lemma}
\begin{proof}
  It follows from \cref{prop:acq-in-cov,prop:rel-fence-in-cov}.
\end{proof}

\begin{lemma}
  $G'.\lSW = G.\lSW; [G'.\lE] \land G'.\lSW = [\CoveredSet]; G'.\lSW; [\CoveredSet]$.
\end{lemma}
\begin{proof}
  Fix $\tup{e, e'} \in G'.\lSW =$ \\
  $[G'.\lE^{\sqsupseteq \rel}]; ([G'.\lF];G'.\lPO)^? ;G'.\lRS;G'.\lRF; (G'.\lPO;[G'.\lF])^?; [G'.\lE^{\sqsupseteq\acq}]$.
  By \cref{prop:acq-in-cov}, $e' \in \CoveredSet$.
  From $\travConfig(G, \tup{\CoveredSet, \IssuedSet})$, it follows that
  $\exists r \in \CoveredSet. \; \tup{e, r} \in [G'.\lE^{\sqsupseteq \rel}]; ([G'.\lF];G'.\lPO)^? ;G'.\lRS;G'.\lRF$.
  We also know that $\tup{r, e'} \in [G.\lR];(G.\lPO;[G.\lF])^?; [G.\lE^{\sqsupseteq\acq}]$.

  From this, we conclude that $\exists w \in \IssuedSet. \; \tup{e, w} \in [G'.\lE^{\sqsupseteq \rel}]; ([G'.\lF];G'.\lPO)^? ;G'.\lRS \land
  \tup{w, r} \in G.\lRF$.
  By the definition of $\lRS$,
  $\tup{e, w} \in [G'.\lE^{\sqsupseteq \rel}]; ([G'.\lF];G'.\lPO)^? ;[\lW]; G'.\lPO\rst\lLOC^? ;
    [\lW];(G'.\lRF;G'.\lRMW)^*$.
  We may simplify the statement--- $\tup{e, w} \in [G'.\lE^{\sqsupseteq \rel}]; G'.\lPO^?;(G'.\lRF;G'.\lRMW)^*$.
  We conclude that $\exists w' \in \IssuedSet. \; \tup{e, w'} \in [G'.\lE^{\sqsupseteq \rel}]; G'.\lPO^? \land \tup{w' ,w} \in (G'.\lRF;G'.\lRMW)^*$.
  From this, we conclude that $e \in \CoveredSet$.
  
  $G.\lSW; [G'.\lE] \suq G'.\lSW$ may be proved in the same way.
\end{proof}

\begin{lemma}
  $G'.\lHB; [\CoveredSet] = G.\lHB; [\CoveredSet]$ and $\dom{G'.\lHB; [\CoveredSet]} = \CoveredSet$.
\end{lemma}
\begin{proof}
  It holds since
  $G'.\lSW = [\CoveredSet]; G.\lSW; [\CoveredSet]$ and
  $G'.\lPO; [\CoveredSet] = G.\lPO; [\CoveredSet] = [\CoveredSet]; G.\lPO; [\CoveredSet]$.
  The latter holds due to $\travConfig(G, \tup{\CoveredSet, \IssuedSet})$.
\end{proof}

\begin{lemma}
  \label{prop:cert-hb-repr}
  $G'.\lHB = G'.\lPO \cup [\CoveredSet]; G.\lHB; [\CoveredSet]; G'.\lPO^?$.
\end{lemma}

\begin{lemma}
  $G'.\lPSC = [G'.\lE]; G.\lPSC; [G'.\lE]$.
\end{lemma}

\begin{lemma}
  \label{prop:currel-cert}
  $G'.\curRel; [\CoveredSet] = G.\curRel; [\CoveredSet]$.
\end{lemma}

\begin{lemma}
  \label{prop:rf-cert-req}
  $G'.\lRF \suq G.\lRF; [D] \cup (G.\curRel; [\CoveredSet])^?; G'.\lPO$.
\end{lemma}
\begin{proof}
  It follows from \cref{prop:currel-cert} and restrictions of $G'.\lRF$ in $\certCompl(G, \tup{\CoveredSet, \IssuedSet}, G')$.
\end{proof}

\begin{lemma}
  $G'.\lHB\rst\lLOC \cup G'.\lRF$ is acyclic.
\end{lemma}
\begin{proof}
  We know that $G'.\lHB \suq G.\lHB$ from \cref{prop:cert-hb-repr}.
  $G'.\lRF \suq G.\lRF \cup ((G.\curRel; [\CoveredSet])^?; G.\lPO)\rst\lLOC$ follows from \cref{prop:rf-cert-req}.
  Their union is acyclic because \ref{ax:scloc} holds for $G$.
\end{proof}


==> mappingLTS.tex <==
\subsection{Mapping Programs to LTS}

%% \newcommand{\DataD}{\Psi_{\sf D}}
%% \newcommand{\CtrlD}{\Omega_{\sf D}}
\newcommand{\DataD}{{\rm Data}}
\newcommand{\CtrlD}{{\rm Ctrl}}
\newcommand{\DepsD}{{\rm Deps}}
\newcommand{\toLts}{{\rm \bf to\text{-}lts}}
\newcommand{\toLtsAux}{{\rm \bf to\text{-}lts\text{-}aux}}
\newcommand{\insertLTS}[2]{#1 \cup \{#2\}}
\newcommand{\tinit}{{\rm t}_{\rm init}}

A transition of thread's state in \Promise has a $label$:
\[\begin{array}{r@{\;}l}
\mathit{label} ::=  & 
\epsilon
\ALT \rlab{o}{x}{v} 
\ALT \wlab{o}{x}{v} 
\ALT \flab{o}
\ALT \ulab{o}{x}{v}{v'}.
\end{array}\]
A transition itself is represented as either an initial transition $\tinit$ or a pair $\tup{transition, label}$:
\[\begin{array}{r@{\;}l}
\mathit{transition} ::=  & 
\tinit \ALT \tup{transition, label}.
\end{array}\]
Semantically, the first component of the pair representing some transition $t$ is a link to a transition which directly precedes
$t$ in a (unique) path, which contains $t$, in LTS.
We use the link to the previous transition to guarantee that a transition uniquely identifies an execution step of a thread.
We need it to be able to define correspondence between transitions and events in execution graphs.

We represent a labeled transition system, $LTS$, as a set of triples $\tup{s, t, s'}$, where $s$ and $s'$ are \emph{states}
and $t$ is a transition. States are represented via pairs $\tup{pc, \Phi}$.
We construct $LTS$ from a thread's list of instructions, $\thr$, via the function $\toLts$.
\[\inarr{
\toLts(\thr) \defeq \toLtsAux(\thr, \tinit, 0, \bot, \bot, \emptyset, \emptyset, \emptyset). \\
}\]
The function returns a pair $\tup{\DepsD, LTS}$, where $\DepsD$ is a relation over transitions used in $LTS$.
The relation $\DepsD$ represents data, address and control dependencies between transitions.

The pairs $\tup{\DepsD, LTS}$ might be combined using an operator $\triangle$:
\[\inarr{
\tup{\DepsD, LTS} \triangle \tup{\DepsD', LTS'} \defeq \tup{\DepsD \cup \DepsD', LTS \cup LTS'}. \\
}\]

%% \app{TODO: add explanation}

%% We define LTS using labels


\[\inarr{
\toLtsAux(\thr, t_{\rm prev}, pc, \Phi,\DataD,\CtrlD, \DepsD, LTS) \defeq \\
\quad \kw{match} \; \thr(pc) \; \kw{with} \\
\quad \ALT \assignInst{r}{e} \to \\
\qquad \letdef{\Phi'}{\Phi[r \mapsto \Phi(e)]} \\
\qquad \letdef{\DataD'}{\DataD[r \mapsto \DataD(e)]} \\
\qquad \letdef{t}{\tup{t_{\rm prev}, \epsilon}} \\
\qquad \letdef{\DepsD'}{(\DataD(e) \cup \CtrlD) \times \{t\}} \\
\qquad \letdef{LTS'}{LTS \cup \{(\tup{pc, \Phi}, t, \tup{pc + 1, \Phi'})\}} \\
\qquad \toLtsAux(\thr, t, pc + 1, \Phi', \DataD', \CtrlD, \DepsD \cup \DepsD', LTS') \\
\\

\quad \ALT \fenceInst{o} \to \\
\qquad \letdef{t}{\tup{t_{\rm prev}, \flab{o}}} \\
\qquad \letdef{\DepsD'}{\CtrlD \times \{t\}} \\
\qquad \letdef{LTS'}{LTS \cup \{\tup{pc, \Phi, t, pc + 1, \Phi}\}} \\
\qquad \toLtsAux(\thr, t, pc + 1, \Phi, \DataD, \CtrlD, \DepsD  \cup \DepsD', LTS') \\
\\

\quad \ALT \writeInst{o}{e_1}{e_2} \to \\
\qquad \letdef{\loc, \val}{\Phi(e_1), \Phi(e_2)} \\
\qquad \letdef{t}{\tup{t_{\rm prev}, \wlab{o}{\loc}{\val}}} \\
\qquad \letdef{\DepsD'}{(\DataD(e_1) \cup \DataD(e_2) \cup \CtrlD) \times \{t\}} \\
\qquad \letdef{LTS'}{LTS \cup \{(\tup{pc, \Phi}, t, \tup{pc + 1, \Phi})\}} \\
\qquad \toLtsAux(\thr, t, pc + 1, \Phi, \DataD, \CtrlD, \DepsD  \cup \DepsD', LTS') \\
}\]

\[\inarr{
\quad \ALT \readInst{o}{r}{e} \to \\
\qquad \letdef{\loc}{\Phi(e)} \\
\qquad \kw{let} \; ltsf \defeq \lambda \val. \{ \\
\qquad \quad \letdef{\Phi'}{\Phi[r \mapsto \val]} \\
\qquad \quad \letdef{t}{\tup{t_{\rm prev}, \rlab{o}{\loc}{\val}}} \\
\qquad \quad \letdef{\DataD'}{\DataD[r \mapsto \DataD(r) \cup \{t\}]} \\
\qquad \quad \letdef{\DepsD'}{(\DataD(e) \cup \CtrlD) \times \{t\}} \\
\qquad \quad \letdef{LTS'}{LTS \cup \{(\tup{pc, \Phi}, t, \tup{pc + 1, \Phi'})\}} \\
\qquad \quad \toLtsAux(\thr, t, pc + 1, \Phi', \DataD', \CtrlD, \DepsD  \cup \DepsD', LTS') \\
\qquad \} \; \kw{in} \\
\qquad \bigtriangleup_{\val \in \Val} ltsf(\val) \\
}\]

%% \quad \ALT \ifGotoInst{e}{n} \; \kw{when} \; \Phi(e) \neq 0 \to \\
%% \qquad \letdef{t}{\tup{pclist, pc, \Phi, \epsilon, n, \Phi}} \\
%% %% \qquad \letdef{\CtrlD'}{\CtrlD \cup \{t\}} \\
%% \qquad \toLtsAux(\thr, n, pc:pclist, \Phi, \DataD, \CtrlD \cup \{t\}, LTS') \\
%% \\

\[\inarr{
\quad \ALT \ifGotoInst{e}{n} \to \\
\qquad \letdef{pc'}{\ite{\Phi(e) \neq 0}{n}{pc + 1}} \\
\qquad \letdef{t}{\tup{t_{\rm prev}, \epsilon}} \\
%% \qquad \letdef{\CtrlD'}{\CtrlD \cup \{t\}} \\
\qquad \letdef{\DepsD'}{(\DataD(e) \cup \CtrlD) \times \{t\}} \\
\qquad \letdef{LTS'}{LTS \cup \{(\tup{pc, \Phi}, t, \tup{pc', \Phi})\}} \\
\qquad \toLtsAux(\thr, t, pc', \Phi, \DataD, \CtrlD \cup \{t\}, \DepsD  \cup \DepsD', LTS') \\
\\
%% }\]

%% \[\inarr{
\quad \ALT \incInst{o_\lR}{o_\lW}{r}{e_1}{e_2} \to \\
\qquad \letdef{\loc, \val'}{\Phi(e_1), \Phi(e_2)} \\
\qquad \kw{let} \; ltsf \defeq \lambda \val. \{ \\
\qquad \quad \letdef{\Phi'}{\Phi[r \mapsto \val]} \\
\qquad \quad \letdef{t}{\tup{t_{\rm prev}, \ulab{o_\lR, o_\lW}{\loc}{\val}{\val + \val'}}} \\
\qquad \quad \letdef{\DataD'}{\DataD[r \mapsto \DataD(e_1) \cup \DataD(e_2) \cup \{t\}]} \\
%% \qquad \quad \letdef{\CtrlD'}{\CtrlD \cup \{ t\}} \\
\qquad \quad \letdef{\DepsD'}{(\DataD(e_1) \cup \DataD(e_2) \cup \CtrlD) \times \{t\}} \\
\qquad \quad \letdef{LTS'}{LTS \cup \{(\tup{pc, \Phi}, t, \tup{pc + 1, \Phi'})\}} \\
\qquad \quad \toLtsAux(\thr, t, pc + 1, \Phi', \DataD', \CtrlD \cup \{ t\}, \DepsD \cup \DepsD', LTS') \\
\qquad \} \; \kw{in} \\
\qquad \bigtriangleup_{\val \in \Val} ltsf(\val) \\
\\

\quad \ALT \casInst{o_\lR}{o_\lW}{r}{e}{e_\lR}{e_\lW} \to \\
\qquad \letdef{\loc, \val_\lR, \val_\lW}{\Phi(e), \Phi(e_\lR), \Phi(e_\lW)} \\
\qquad \kw{let} \; ltsf \defeq \lambda \val. \{ \\
\qquad \quad
  \iteml{\val = \val_\lR}{
\letdef{\Phi'}{\Phi[r \mapsto \val_\lR]} \\
\letdef{t}{\tup{t_{\rm prev}, \ulab{o_\lR, o_\lW}{\loc}{\val_\lR}{\val_\lW}}} \\
\letdef{\DataD'}{\DataD[r \mapsto \DataD(e) \cup \DataD(e_\lR) \cup \DataD(e_\lW) \cup \{t\}]} \\
\letdef{\DepsD'}{(\DataD(e) \cup \DataD(e_\lR) \cup \DataD(e_\lW) \cup \CtrlD) \times \{t\}} \\
\letdef{LTS'}{LTS \cup \{(\tup{pc, \Phi}, t, \tup{pc + 1, \Phi'})\}} \\
\toLtsAux(\thr, t, pc + 1, \Phi', \DataD', \CtrlD \cup \{ t\}, \DepsD \cup \DepsD', LTS') \\
  }{
\letdef{\Phi'}{\Phi[r \mapsto \val]} \\
\letdef{t}{\tup{t_{\rm prev}, \rlab{o_\lR}{\loc}{\val}}} \\
\letdef{\DataD'}{\DataD[r \mapsto \DataD(e) \cup \DataD(e_\lR) %\cup \DataD(e_\lW)
    \cup \{t\}]} \\
\letdef{\DepsD'}{(\DataD(e) \cup \DataD(e_\lR) \cup \CtrlD) \times \{t\}} \\
\letdef{LTS'}{LTS \cup \{(\tup{pc, \Phi}, t, \tup{pc + 1, \Phi'})\}} \\
\toLtsAux(\thr, t, pc + 1, \Phi', \DataD', \CtrlD \cup \{ t\}, \DepsD \cup \DepsD', LTS') \\
  }
  \\
\qquad \} \; \kw{in} \\
\qquad \bigtriangleup_{\val \in \Val} ltsf(\val) \\
\\

\quad \ALT \bot \to \{\tup{\DepsD, LTS}\}.
}\]

In our simulation proof, we need to show that the \Promise machine may certify its steps.
To do so, we construct a ``certification'' graph $G'$ from the \PH execution $G$,
which the \Promise machine tries to simulate (see \cref{sec:cert}).
The ``certification'' graph $G'$ is a $\lPO$-prefix of some \PH execution of the same program (see $\prefix$ in \cref{sec:cert}).
$G'$ might be obtained from $G$ by dropping $\lPO$-suffix of the execution (\ie events which don't precede issued writes)
and by modifying some events and relations on them (see $\certCompl$ in \cref{sec:cert}).
More specifically, we modify each read event $r$ (and all subsequent events which depend on it), which isn't
in $\dom{(G.\lDEPS \cup G.\lRFI)^+; [\IssuedSet]}$, 
to read from the $\lMO$-latest write event in $\dom{\curRel; [r]}$.
Here $\IssuedSet$ is a set of issued writes.
%% \ie, in terms of \Promise, the message with a timestamp equal to the corresponding value of thread's$\viewCur(\lLOC(r))$.

To be able to simulate the ``certification'' graph $G'$, we have to show that LTS allows the same modifications.
The requirement is stated in \cref{thm:cert-lts}. In the theorem, we have a universally quantified relation on transitions, $R$,
which is instantiated correspondingly to $G'.\lRFI$, when the theorem is used in simulation of $G'$.
\begin{theorem}
  \label{thm:cert-lts}
\[\inarr{
  \forall \thr, \tup{\DepsD, LTS} = \toLts(\thr), n, S = \{s_i\}_{i \in [0..n]}, T = \{t_i\}_{i \in [0..n)}, W \suq T, R. \\
  \quad (\forall i \in [0..n). \; (s_i, t_i, s_{i+1}) \in LTS) \land {} \\
  \quad {\rm is\_read}(t_0) \land [t_0]; (\DepsD \cup R)^{+}; [W] = \emptyset \Rightarrow \\
  \qquad \forall t'_0 \approx t_0. \; \exists S' = \{s'_i\}_{i \in [0..n]}, T' = \{t'_i\}_{i \in [0..n)}. \\
  \qquad \quad s_0 = s'_0 \land (\forall i \in [0..n). \; (s'_i, t'_i, s'_{i+1}) \in LTS) \land
    (\forall i. \; t_i \in W \Rightarrow t'_i = t_i).
}\]
\end{theorem}

In the theorem's formulation, we use an operator $\approx$:
\[\inarr{
  t \approx t' \defeq \\
  \quad \kw{match} \; t, t' \; \kw{with} \\
  \quad \ALT \tinit, \tinit \Rightarrow True \\
  \quad \ALT \tup{t'', lab}, \tup{t'', lab'} \Rightarrow \\
  \qquad \kw{match} \; lab, lab' \; \kw{with} \\
  \qquad \ALT \epsilon, \epsilon
         \ALT \rlab{o}{x}{\_}, \rlab{o}{x}{\_}
         \ALT \wlab{o}{x}{\_}, \wlab{o}{x}{\_} \\
  \qquad \ALT \ulab{o_\lR, o_\lW}{x}{\_}{\_}, \ulab{o_\lR, o_\lW}{x}{\_}{\_}
         \ALT \flab{o}, \flab{o} \Rightarrow True \\
  \qquad \ALT \_ \Rightarrow False \\
  \quad \ALT \_ \Rightarrow False.
}\]



==> oldIHs.tex <==
\subsection{The intermediate model \IMMs}
\label{sec:S_IH}
In our simulation proof, we want to have a close connection between views of the \Promise machine
and graph executions. 

%% For an execution, $G$, we therefore define the following relations:
\begin{align*}
 \lRSs &\defeq [\lW];\lPO\rst\lLOC;[\lW];(\lRF;\lRMW)^*
 \tag{\emph{release sequence}} \\
 \lRELEASEs &\defeq [\lE^{\sqsupseteq \rel}]; ([\lF];\lPO)^? ;\lRSs
 \tag{\emph{release prefix}} \\
 \lSWs &\inarr{{}\defeq  \lRELEASEs; \lRF; (\lPO;[\lF])^?; [\lE^{\sqsupseteq\acq}]} 
 \tag{\emph{synchronizes with}} \\
 \lHBs &\defeq (\lPO \cup \lSWs)^+ \tag{\emph{happens-before}}  \\
 \\
 \lPSCs &\defeq [\lF^\sco] ;\lHBs; \lECO;\lHBs; [\lF^\sco] \tag{\emph{partial SC-fence order}} \\
 \lARs &\defeq \lAR \setminus \lPSC \cup \lPSCs \\
\end{align*}

\begin{definition}
\label{def:smodel}
An extended execution $G$ is called \emph{\IMMs-consistent} if the following hold:
\begin{itemize}
\item $G.\lHBs;\lECO^?$ is irreflexive. \labelAxiom{s-coherence}{ax:coh}
\item $G.\lRMW \cap (G.\lFRE;G.\lCOE) = \emptyset$.  \labelAxiom{s-atomicity}{ax:at}
\item $G.\lARs$ is acyclic. \labelAxiom{s-no-thin-air}{ax:nta}
\end{itemize}
\app{TODO: say something about $\lSC$}
\end{definition}

\begin{proposition}
  \label{ph-to-phs}
  Let $G$ be a \IMM-consistent execution. Then, $G$ is \IMMs-consistent.
\end{proposition}
\begin{proof}[Proof outline]
  From definitions it follows that $G.\lRSs \suq G.\lRS$, $G.\lSWs \suq G.\lSW$, $G.\lHBs \suq G.\lHB$,
  $G.\lPSCs \suq G.\lPSC$, and $G.\lARs \suq G.\lAR$.
  Thus, from irreflexivity of $G.\lHB;\lECO^?$ it follows that $G.\lHBs;\lECO^?$ is irreflexive, and
  from acyclicity of $G.\lAR$ it follows that $G.\lARs$ is acyclic.
\end{proof}
\cref{ph-to-phs} allows to get correctness of compilation from \Promise to \IMM by proving correctness of compilation from
\Promise to \IMMs.

